Driving Through Uncertainty: Risk-Averse Control with LLM Commonsense for Autonomous Driving under Perception Deficits

Partial perception deficits can compromise autonomous vehicle safety by disrupting environmental understanding. Existing protocols typically default to entirely risk-avoidant actions such as immediate stops, which are detrimental to navigation goals and lack flexibility for rare driving scenarios. Yet, in cases of minor risk, halting the vehicle may be unnecessary, and more adaptive responses are preferable. In this paper, we propose LLM-RCO, a risk-averse framework leveraging large language models (LLMs) to integrate human-like driving commonsense into autonomous systems facing perception deficits. LLM-RCO features four key modules interacting with the dynamic driving environment: hazard inference, short-term motion planner, action condition verifier, and safety constraint generator, enabling proactive and context-aware actions in such challenging conditions. To enhance the driving decision-making of LLMs, we construct DriveLM-Deficit, a dataset of 53,895 video clips featuring deficits of safety-critical objects, annotated for LLM fine-tuning in hazard detection and motion planning. Extensive experiments in adverse driving conditions with the CARLA simulator demonstrate that LLM-RCO promotes proactive maneuvers over purely risk-averse actions in perception deficit scenarios, underscoring its value for boosting autonomous driving resilience against perception loss challenges.

==> tabs/constraint_factors.tex <==
\begin{table}[!htbp]
  \centering
  \resizebox{7cm}{!}
  {
      \begin{tabular}{@{}lc@{}}
        \toprule
        Factor & Values \\
        \midrule
        Weather & \makecell{Cloudy, Wet, MidRain, WetCloudy, \\ HardRain, SoftRain} \\
        Daylight & Night, Noon, Sunset, Dawn, Morning, Twilight \\
        Road Geometry & \makecell{Straight, Intersection-3Way, Intersection-4Way, \\ Roundabout, Ramp, One-Way}\\
        Direction & TurnLeft, TurnRight, Straight\\
        Traffic Env & City, Suburban, Rural, HighWay\\
        Traffic Density & High, Medium, Low \\
        \bottomrule
      \end{tabular}
  }
  \caption{Factors for autonomous driving safety control constraints.}
  \label{tab:factors}
\end{table}

==> tabs/drop_visionloss.tex <==
\begin{table*}[!htbp]
  \centering
  \resizebox{\textwidth}{!}
  {
      \begin{tabular}{llcccccccc}
      \toprule 
       \multirow{2}{*}{\textbf{Agent}} & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{8}{c}{\textbf{Adverse Conditions}} \\
       \cmidrule{3-10}
       & & Traffic Light & Traffic Sign & Pedestrian & Motorcycle & MaskC50 & MaskC100 & MaskTF50 & MaskTF100  \\
        \midrule
        \multirow{3}{*}{Transfuser} & RC$\uparrow$ &&&&&&&& \\
        & IS$\uparrow$ &&&&&&&& \\
        & DS$\uparrow$ &&&&&&&& \\
        \midrule
        \multirow{3}{*}{Interfuser} & RC$\uparrow$ & 46.88\pm7.21$\downarrow$ & 46.97\pm5.33$\downarrow$& & & 4.67\pm0.24$\downarrow$ & 11.4\pm0.59$\downarrow$ & 3.12\pm0.66$\downarrow$ & 7.81\pm0.50$\downarrow$ \\
        & IS$\uparrow$ & 0.51\pm0.14$\downarrow$ & & & & 0.12\pm0.04$\downarrow$ & 0.50\pm0.11$\downarrow$& 0.02\pm0.01$\downarrow$ & 0.14\pm0.06$\downarrow$ \\
        & DS$\uparrow$ & 26.03\pm7.45$\downarrow$ & & & & 10.97\pm2.15$\downarrow$ & 29.63\pm3.54$\downarrow$& 5.11\pm2.17$\downarrow$& 19.18\pm6.72$\downarrow$ \\
      \bottomrule   
      \end{tabular}
  }
  \caption{Table.}
  \vspace{-3mm}
  \label{tab:drop}
\end{table*}

==> tabs/overall_result_mask.tex <==
\begin{table}[!htbp]

  \centering
  \resizebox{0.45\textwidth}{!}{
      \begin{tabular}{ccccccccc}
      \toprule 
       \multirow{2}{*}{\textbf{Experiment}} & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{2}{c}{Top-Left} & \multicolumn{2}{c}{Center} & \multicolumn{2}{c}{Bottom-Right} \\
       \cmidrule{3-8}
        & & TF & IF & TF & IF & TF & IF  \\
        \midrule
        \rowcolors{3}{gray!15}{white}
        \multirow{3}{*}{\makecell{\textbf{Visual Deficit} \\ LLM-RCO \textcolor{red}{\ding{55}} }} & RC$\uparrow$ & - & - & - & - & - & - \\
        & IS$\uparrow$ & - & - & - & - & - & -  \\
        & DS$\uparrow$ & - & - & - & - & - & -  \\
        \hline  
        \multirow{3}{*}{\makecell{\textbf{Visual Deficit} \\ LLM-RCO \textcolor{green}{\ding{51}} \\ HI-GPT,STP-GPT }} & RC$\uparrow$ & - & - & - & - & - & - \\
        & IS$\uparrow$ & - & - & - & - & - & -  \\
        & DS$\uparrow$ & - & - & - & - & - & -  \\
         \hline
        \multirow{3}{*}{\makecell{\textbf{Visual Deficit} \\ LLM-RCO \textcolor{green}{\ding{51}} \\ HI-Qiwen,STP-GPT}} & RC$\uparrow$ & - & - & - & - & - & -  \\
        & IS$\uparrow$ & - & - & - & - & - & -  \\
        & DS$\uparrow$ & - & - & - & - & - & -  \\
      \bottomrule   
      \end{tabular}
  }
  \caption{Comparison of driving metrics w/o visual deficits and w/o LLM-RCO control override across various perception deficit scenarios.}
  \vspace{-3mm}
  \label{tab:overall}
\end{table}
